Agentic discovery of blood biomarker from distilled private health records

Routine complete blood counts (CBCs) could yield new biomarkers, but the private records needed to evaluate candidates cannot be shared with frontier language model agents that excel at discovery. We distilled the evidence held in the Clalit Health Services panel of over 5.4 million patients into a released scoring tool: for each of 13 immune-mediated diseases, a graph attention network was trained inside the data boundary to predict the case-control AUC of candidate CBC expressions, and only the trained weights were released. The tool grounds an agent's propose-score-refine loop in real-world data without exposing any patient data. In external validation, agent-discovered expressions improved on their literature-seeded starting points by a median of 4.18 AUC percentage points, and across three independent cohorts, reranking the candidates of three frontier research tools improved on their first choices in most comparisons, with gains that varied by cohort. The released scorer supports privacy-preserving biomarker hypothesis generation.

==> biomarker_shapley_verdicts_table.tex <==
\begin{table}[!ht]
\centering\footnotesize
\caption{Shapley attribution of each discovered biomarker's components and their concordance with the clinical literature. For every disease, each blood-count feature in the discovered expression is attributed a signed Shapley contribution to the out-of-sample MIMIC-IV disease prediction, then classified against the literature as \emph{Expected} (model direction matches the established association), \emph{Surprising} (contradicts it or has no recognised link), or \emph{Unclear}. Arrows give the model direction of the dominant driver ($\uparrow$/$\downarrow$ = higher level raises/lowers predicted risk). AUC is the primary-cohort (MIMIC-IV) value of Table~\ref{tab:discovered_main}. Full per-feature verdicts and verified citations are in Supplementary Data~1. (LYM\%, NEUT\%, EOS\% and BASO\% denote the LYMpct/NEUTpct/EOS\_pct/BASO\_pct features of Table~\ref{tab:discovered_main}.)}
\label{tab:shapley_verdicts}
\begin{tabular}{llccl l}
\toprule
\textbf{Disease (ICD)} & \textbf{AUC} & \textbf{Exp.} & \textbf{Surp.} & \textbf{Dominant driver} & \textbf{Notable surprising} \\
\midrule
Systemic lupus (SLE) (7100) & 0.676 & 6 & 0 & WBC~$\downarrow$ & --- \\
Rheumatoid arthritis (714) & 0.615 & 5 & 1 & RDW~$\uparrow$ & MCHC~$\downarrow$ \\
Hashimoto thyroiditis (2452) & 0.606 & 3 & 2 & LYM\%~$\uparrow$ & LYM\%~$\uparrow$, HCT~$\uparrow$ \\
Hyperthyroidism (242) & 0.602 & 4 & 1 & HB~$\downarrow$ & RDW~$\uparrow$ \\
Psoriasis (696) & 0.597 & 4 & 4 & EOS\%~$\uparrow$ & BASO\%~$\uparrow$, HB~$\uparrow$, \ldots \\
Sj\"ogren's syndrome (7102) & 0.596 & 4 & 1 & RDW~$\uparrow$ & MCV~$\uparrow$ \\
Systemic sclerosis (7101) & 0.588 & 4 & 1 & RDW~$\uparrow$ & MCV~$\uparrow$ \\
Ulcerative colitis (556) & 0.572 & 1 & 5 & LYM\%~$\uparrow$ & LYM\%~$\uparrow$, HB~$\uparrow$, \ldots \\
Crohn's disease (555) & 0.570 & 5 & 0 & LYM\%~$\downarrow$ & --- \\
Multiple sclerosis (340) & 0.570 & 0 & 3 & NEUT\%~$\downarrow$ & NEUT\%~$\downarrow$, HB~$\uparrow$, \ldots \\
Type 1 diabetes (250) & 0.568 & 3 & 3 & LYM\%~$\downarrow$ & WBC~$\uparrow$, RDW~$\uparrow$, \ldots \\
Celiac disease (5790) & 0.557 & 2 & 0 & RBC~$\downarrow$ & --- \\
\midrule
\textbf{All 12 (64 components)} & --- & \textbf{41} & \textbf{21} & \multicolumn{2}{l}{2 Unclear; anaemia-of-inflammation axis dominant} \\
\bottomrule
\end{tabular}
\end{table}

